Distal combinatorial tools for graphs of bounded twin-width

We study set systems formed by neighborhoods in graphs of bounded twin-width. We start by proving that such graphs have linear neighborhood complexity, in analogy to previous results concerning graphs from classes with bounded expansion and of bounded clique-width. Next, we shift our attention to the notions of distality and abstract cell decomposition, which come from model theory. We give a direct combinatorial proof that the edge relation is distal in classes of ordered graphs of bounded twin-width. This allows us to apply Distal cutting lemma and Distal regularity lemma, so we obtain powerful combinatorial tools for graphs of bounded twin-width.

==> distality.tex <==
\section{Combinatorial tools for graphs of bounded twin-width}
\label{chap:tools}
In this Section we derive powerful combinatorial consequences of Theorem \ref{theorem:encoding_theorem}  proved in the previous section.
Namely, we observe that our theorem implies that ordered graphs of bounded twin-width allow \emph{abstract cell decompositions} studied in model theory \cite{distal}. Combining with results 
from \cite{distal} and \cite{regularity}, this yields immediate powerful structural properties of graphs of bounded twin-width,
such as the Distal cutting lemma and the Distal regularity lemma.
We start this section with a few more definitions related to logic and model theory.

\subsection{Definition of twin-width of matrices and binary structures}
\label{subsec:twin_width_bin_structs}
The twin-width is also defined in \cite{twinwidth1} for matrices that have entries over a finite alphabet with a special additional value $r$ (for red) representing errors made along the computation.
The red number of a matrix is the maximum number of red entries taken over all rows and all columns.
Given an $m \times n$ matrix $M$ and two columns $C_i$ and $C_j$, the contraction of $C_i$ and $C_j$ is obtained by deleting $C_j$ and replacing every entry $M[k][i]$ of $C_i$ by $r$ whenever $M[k][i] \neq M[k][j]$.
The same contraction operation is defined for rows.

A matrix M has twin-width at most $k$ if one can perform a sequence of contractions starting with $M$ and ending in some $1 \times 1$ matrix in such a way that all matrices occurring in the process have red number at most $k$.
Note that when $M$ has twin-width at most $k$, one can reorder its rows and columns in such a way that every contraction will identify consecutive rows and columns.
The reordered matrix is then called \emph{$k$-twin-ordered}.

The \emph{symmetric twin-width} of an $n \times n$ matrix $M$ is defined similarly, except that the contraction of rows $i$ and $j$ (resp. columns $i$ and $j$) is immediately followed by the contraction of columns $i$ and $j$ (resp. rows $i$ and $j$).
Again, if $M$ has symmetric twin-width at most $k$, we can reorder its rows and columns in such a way that every contraction will identify consecutive rows and columns.
The reordered matrix is then called \emph{$k$-symmetric-twin-ordered}.

For a binary structure $\Ss$ with a domain $S = \set{\seq vn}$ over $h$ binary relations $E^1, \ldots E^h$ we build its adjacency matrix $M$ in such a way that $M[i][j] = (\seq eh) \in \set{-1, 0, 1, 2}^h$ where every $e_p$ is chosen accordingly.
Namely:
\begin{itemize}
    \item if $E^p(v_i, v_j)$ and $E^p(v_j, v_i)$ we set $e_p = 2$;
    \item if $E^p(v_i, v_j)$ and $\neg  E^p(v_j, v_i)$ we set $e_p = 1$;
    \item if $\neg E^p(v_i, v_j)$ and $E^p(v_j, v_i)$ we set $e_p = -1$;
    \item if $\neg E^p(v_i, v_j)$ and $ \neg E^p(v_j, v_i)$ we set $e_p = 0$.
\end{itemize}
The twin-width of a binary structure is the symmetric twin-width of the so-built adjacency matrix.

Let us assume that for some binary structure $\Ss$ there is a total order $\sigma$ on $S$ such that the adjacency matrix of $\Ss$ in this order is $k$-symmetric-twin-ordered.
It is straightforward to see, that if we add $\sigma$ to $\Ss$ as a new binary relation $E^{h+1}$ (thus obtaining a new structure $\Ss^+$), then the adjacency matrix of $\Ss^+$ in order $\sigma$ is still $k$-symmetric-twin-ordered.

Observe, that whenever a graph $G$ has twin-width at most $t$ in the sense of definition in Section \ref{subsec:twin_width_graphs_def} then its twin-width as a binary structure in the sense of this definition is at most $t + 2$.
Let $\preceq$ be a total order on $V(G)$ such that the adjacency matrix of $G$ with rows and columns ordered by $\preceq$ is $(t + 2)$-symmetric-twin-ordered.
We clearly see that the binary structure $(G, \preceq)$ with two binary relations $E$ and $\preceq$ also has twin-width at most $t + 2$.
Moreover, by \cite[Theorem 10]{twinwidth1} we obtain that $M_\preceq(G)$ it $2t + 6$-mixed free.
For a graph $G$ of twin-width at most $t$ we call a total order $\preceq$ on its vertices, that satisfies properties above, a \emph{$t$-proper order} for $G$.

\subsection{Infinite model of all graphs of twin-width bounded by a fixed integer}
For the rest of this section fix $\Sigma$ and $\Pi$ to be binary relational signatures $\set{E, \preceq}$ and $\set{E, \preceq, \hpreceq}$ respectively.
We already observed in Section \ref{subsec:twin_width_bin_structs} that for any graph $G$ of twin-width at most $t$ we can find a $t$-proper total order on its vertices~$\preceq$ (i.e. $M_\preceq(G)$ is $2t+6$-mixed free and $(G, \preceq)$ seen as a binary $\Sigma$-structure has twin-width bounded by $t+2$).
Sometimes, by abuse of notation, we will denote $\preceq$ for a binary structure $(G, \preceq)$ by $\preceq_G$ to avoid confusion with $\preceq$ on other structures.
We will do the same for the edge relation $E_G$.

For a fixed integer $t$, let $\Cc_t$ be the class of all (up to isomorphism) finite $\Sigma$-structures $(G, \preceq_G)$ such that $\preceq$ is a $t$-proper order for $G$.
We may assume that for any $(G, \preceq_G) \in \Cc_t$ we have $V(G) \subset \N$ and for any distinct $(G, \preceq_G), (G', \preceq_{G'}) \in \Cc_t$ their vertex sets are disjoint.
We also assume that $\Cc_t = \set{(G_1, \preceq_{G_1}), (G_2, \preceq_{G_2}), \ldots}$, i.e. graphs in $\Cc_t$ are ordered by natural numbers.
%From the definition of twin-width of a binary structure clearly follows, that a disjoint union of any finite subset of $\Cc_t$ is a binary structure with twin-width at most $t+2$.

Let $\M_t$ be the infinite $\Pi$-structure that is the disjoint sum of all structures in $\Cc_t$ together with the total order $\hpreceq$ on its universe, which is consistent with the order of graphs in $\Cc_t$.
Formally, the domain $M_t$ of $\M_t$ is the sum of all vertex sets of structures in $\Cc_t$ (i.e. $M_t = \bigcup_{(G, \preceq_G) \in \Cc_t} V(G)$), and:
\begin{itemize}
    \item for any $x, y \in M_t$ we have $E(x, y)$ if and only if there is a $(G, \preceq_G) \in \Cc_t$ such that $x, y \in V(G)$ and $E_G(x, y)$;
    \item for any $x, y \in M_t$ we have $x \preceq y$ if and only if there is a $(G, \preceq_G) \in \Cc_t$ such that $x, y \in V(G)$ and $x \preceq_G y$;
    \item for any $x, y \in M_t$ we have $x \hpreceq y$ if and only if there are $(G_i, \preceq_{G_i}), (G_j, \preceq_{G_j}) \in \Cc_t$ such that $x \in V(G_i)$, $y \in V(G_j)$ and either $i < j$ or it holds that $i = j$ and $x \preceq_{G_i} y$.
\end{itemize}

By Theorem \ref{theorem:neighborhood-complexity-theorem} for every integer $t$ there is some constant $k$ such that for every graph $G$ of twin-width at most $t$ and for all vertices $a_i \in V(G) (i \in [l])$ and $b_I \in V(G) (I \subseteq [l])$ if
\[
    E(a_i, b_I) \iff i \in I,
\]
then $l \le k$.
Indeed, the negation of this statement would contradict the fact, that classes of graphs of bounded twin-width admit linear neighborhood complexity.

Using this fact and \cite[Theorem 39]{twinwidth1} we can prove the following lemma.
\begin{restatable}{lemma}{mtisnip}
\label{lemma:m_t_is_nip}
    For every integer $t$ the structure $\M_t$ is monadically NIP.
\end{restatable}

The proof of Lemma \ref{lemma:m_t_is_nip} is rather simple but technical, so we defer it to Appendix \ref{appendix:nip}.

Now we show another property of $\M_t$ -- the edge relation in this structure admits a definable abstract cell decomposition.

\begin{theorem}
\label{lemma:abstract_cell_decomposition_for_m_t}
    For any integer $t$ formula $\phi(x, y) \equiv E(x, y)$ admits a definable abstract cell decomposition $\T$ in the structure $\M_t$, such that for any finite $S \subset M_t$ we have $|\T(S)| = |S|^{O(t)}$.
\end{theorem}
\begin{proof}
    We know that the formula $\psi_t$ from Proposition \ref{prop:encoding_for_cell_decomposition} gives a weakly definable abstract cell decomposition $\T'$ of $\phi$ for any ordered graph $(G, \preceq) \in \Cc_t$.
    Therefore, for any $G_i$ such that $A = S \cap V(G_i) \neq \emptyset$ we can directly use $\psi_t$ to partition $V(G_i)$ into subsets with the same neighborhood in $S$ using parameters from $A$.
    It remains to split into definable sets the vertices of $G_j$'s such that $S \cap V(G_j) = \emptyset$.
    This can be easily done by using pairs of elements $s_k, s_l \in S$ such that $s_k \hpreceq s_l$ and no other element from $S$ is between $s_k$ and $s_l$ in $\hpreceq$.
    Indeed, we just define sets of vertices that are between such pairs $s_k, s_l$ in $\hpreceq$ and are not in $\preceq$ relation neither with $s_k$ nor with $s_l$.
    
    %Indeed, it follows from the fact, that for any $v \in M_t$ using the relation $\preceq$ we can find all the vertices of the ordered graph $(G, \preceq_G) \in \C_t$ such that $v \in V(G)$.
    %Therefore, for any finite set $S \in M_t$ we can just apply Proposition \ref{prop:encoding_for_cell_decomposition} to the ordered graph $(G, \preceq_G)$ with $A = S \cap V(G)$.
    
    By remark in Section \ref{subsec:abstract_cell_decompositions}, there is also a definable abstract cell decomposition $\T = \T'^{\max}$ weakly definable by the formulas, we described.
    As they have $O(t)$ parameters, we have that for any finite $S \subset M_t$ the condition $|\T(S)| = |S|^{O(t)}$ holds.
\end{proof}

Lemmas \ref{lemma:m_t_is_nip} and \ref{lemma:abstract_cell_decomposition_for_m_t} allow us to derive a number of combinatorial tools known for distal structures for graphs of bounded twin-width.
A structure is \emph{distal} if every formula $\phi(\bar x, \bar y)$ admits a definable abstract cell decomposition.
Although we did not show that $\M_t$ is distal, we know that edge relation in $\M_t$ admits definable abstract cell decomposition.
That is enough to formulate these tools.

\subsection{Cutting lemma for graphs of bounded twin-width}
By simple application of \cite[Theorem 3.2]{distal} to $\M_t$ we obtain the following theorem.
\begin{theorem}
    For any fixed integer $t$ there exists a constant $C = C(t)$, such that for any $(G, \preceq) \in \Cc_t$, any $A \subseteq V(G)$ of size $n$ and any real $r$ satisfying $1 \le r \le n$ we can partition $V(G)$ into sets $\seq Xl$ with
    \[
        l \le Cr^{O(t)},
    \]
    such that for every $X_i$ there are at most $\frac nr$ vertices in $a \in A$ for which $N_{X_i}(a)$ crosses $X_i$ (i.e. there are vertices $x, x' \in X_i$ satisfying $E(x, a)$ and $\neg E(x', a)$).
    Moreover, each of the $X_i$'s is an intersection of at most two $\psi_t(x; A)$ definable sets.
\end{theorem}

% \subsection{Strong Erdős-Hajnal property for graphs of bounded twin-width}
% By repeating the proof of \cite[Theorem 3.1.]{regularity} and applying it to $\M_t$ we can also show, that graphs of bounded twin-width have the strong Erdős-Hajnal property in a definable way.

% \begin{theorem}
% \label{theorem:erdos_hajnal}
%     For any fixed integer $t$ there are a constant $\delta = \delta(t) > 0$ and a pair of formulas $\theta_1(x; \bar {z_1}), \theta_2(x; \bar {z_2})$ such that for any graph $(G, \preceq) \in \C_t$ and any two subsets of its vertices $A, B \subseteq V(G)$, there are two tuples $\bar {c_1} \in V(G)^{|\bar {z_1}|}, \bar {c_2} \in V(G)^{|\bar {z_2}|}$ that define homogeneous sets $A' = \theta_1(G; \bar {c_1}) \subseteq A$ and $B' = \theta_2(G; \bar {c_2}) \subseteq B$ satisfying $|A'| \ge \delta |A|$, $|B'| \ge \delta |B|$.
% \end{theorem}

\subsection{Regularity lemma for graphs of bounded twin-width}
By repeating the proof of \cite[Theorem 5.8]{regularity} and applying it to $\M_t$ we obtain a strong regularity lemma for graphs of bounded twin-width.

\begin{restatable}{theorem}{regularitylemma}
\label{theorem:regularity_lemma}
    For any fixed integer $t$ and any $\epsilon > 0$ there are a constant $c = c(t)$ and $K = O_t((\frac 1\epsilon)^c)$ such that for any graph $G$ of twin-width at most $t$ there is a partition $\seq PK$ of vertices of $G$, such that
    \[
        \sum |P_i||P_j| \le \epsilon |V(G)|^2
    \]
    where the sum is over all $i, j \in [|V(G)|]$ such that $P_i$ and $P_j$ are not homogeneous.
\end{restatable}

